EventKG+Click: A Dataset of Language-specific Event-centric User Interaction Traces

An increasing need to analyse event-centric cross-lingual information calls for innovative user interaction models that assist users in crossing the language barrier. However, datasets that reflect user interaction traces in cross-lingual settings required to train and evaluate the user interaction models are mostly missing. In this paper, we present the EventKG+Click dataset that aims to facilitate the creation and evaluation of such interaction models. EventKG+Click builds upon the event-centric EventKG knowledge graph and language-specific information on user interactions with events, entities, and their relations derived from the Wikipedia clickstream.

==> tables_backup.tex <==
\begin{table}
\center
\caption{Correlations of influence factors with entity click counts and entity relevance scores in \dataset{}. For example, there is a correlation coefficient of $TODO$ between the German entity relevance score and the German event \textit{Location} closeness influence factor.}
\label{tab:entity_correlations}
\begin{tabular}{ll|c|r|r|r|r|r|l|c|r|r|r|r|r|}
\cline{3-8} \cline{10-15}
 &  & \multicolumn{6}{c|}{\textbf{Click Counts}} &  & \multicolumn{6}{c|}{\textbf{Relevance Scores}} \\ \cline{3-8} \cline{10-15} 
 &  & \multicolumn{3}{c|}{\textbf{\textit{Location}}} & \multicolumn{3}{c|}{\textbf{\textit{Links}}} &  & \multicolumn{3}{c|}{\textbf{\textit{Location}}} & \multicolumn{3}{c|}{\textbf{\textit{Links}}} \\ \cline{3-8} \cline{10-15} 
 &  & \textbf{\en} & \multicolumn{1}{c|}{\textbf{\de}} & \multicolumn{1}{c|}{\textbf{\ru}} & \multicolumn{1}{c|}{\textbf{\en}} & \multicolumn{1}{c|}{\textbf{\de}} & \multicolumn{1}{c|}{\textbf{\ru}} &  & \textbf{\en} & \multicolumn{1}{c|}{\textbf{\de}} & \multicolumn{1}{c|}{\textbf{\ru}} & \multicolumn{1}{c|}{\textbf{\en}} & \multicolumn{1}{c|}{\textbf{\de}} & \multicolumn{1}{c|}{\textbf{\ru}} \\ \cline{1-1} \cline{3-8} \cline{10-15} 
\multicolumn{1}{|c|}{\textbf{\en}} &  & \multicolumn{1}{r|}{} &  &  &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  \\ \cline{1-1} \cline{3-8} \cline{10-15} 
\multicolumn{1}{|c|}{\textbf{\de}} &  & \multicolumn{1}{r|}{} &  &  &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  \\ \cline{1-1} \cline{3-8} \cline{10-15} 
\multicolumn{1}{|c|}{\textbf{\ru}} &  & \multicolumn{1}{r|}{} &  &  &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  \\ \cline{1-1} \cline{3-8} \cline{10-15} 
\end{tabular}
\end{table}
